Frequency Enhanced Pre-training for Cross-city Few-shot Traffic Forecasting

The field of Intelligent Transportation Systems (ITS) relies on accurate traffic forecasting to enable various downstream applications. However, developing cities often face challenges in collecting sufficient training traffic data due to limited resources and outdated infrastructure. Recognizing this obstacle, the concept of cross-city few-shot forecasting has emerged as a viable approach. While previous cross-city few-shot forecasting methods ignore the frequency similarity between cities, we have made an observation that the traffic data is more similar in the frequency domain between cities. Based on this fact, we propose a \textbf{F}requency \textbf{E}nhanced \textbf{P}re-training Framework for \textbf{Cross}-city Few-shot Forecasting (\textbf{FEPCross}). FEPCross has a pre-training stage and a fine-tuning stage. In the pre-training stage, we propose a novel Cross-Domain Spatial-Temporal Encoder that incorporates the information of the time and frequency domain and trains it with self-supervised tasks encompassing reconstruction and contrastive objectives. In the fine-tuning stage, we design modules to enrich training samples and maintain a momentum-updated graph structure, thereby mitigating the risk of overfitting to the few-shot training data. Empirical evaluations performed on real-world traffic datasets validate the exceptional efficacy of FEPCross, outperforming existing approaches of diverse categories and demonstrating characteristics that foster the progress of cross-city few-shot forecasting.

==> table/ablation_bkp.tex <==
\begin{table*}[htb]
% \caption{Performance comparison between FDTI and baselines on four datasets. All attention based methods can not run on these large scale datasets and AGCRN, as can not run on the first three datasets due to the unrealistically huge memory consumption. Horizon means the number of forecasting steps.}
% \vspace{-.1cm}
\caption{Overall performance of few-shot traffic forecasting on \textit{PEMS-BAY}, \textit{METR-LA}, \textit{Chengdu}, and \textit{Shenzhen}. Metr-LA$\rightarrow$PEMS-BAY means the source data is METR-LA and the target data is PEMS-BAY. The mean and standard deviation of the results in 5 runs is shown. In each column, the best result is highlighted in bold and grey, and the second-best result is underlined. Marker * and ** indicates the mean of the results is statistically significant  (* means t-test with p-value $<$ 0.05 and ** means t-test with p-value $<$ 0.01). M means using momentum method to update adjacency matrix for STmodel. S means using spatial layer in transformer encoder. E means using augmented data during finetuning. C means using contrastive loss in pretrain.}
\label{tab:ablation_bkp}
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{c|c c|c c|c c||c c|c c|c c}
\resizebox{0.99\linewidth}{!}{

\begin{tabular}{c|c c c c c c||c c c c c c}
\toprule
& \multicolumn{6}{c||}{\textbf{METR-LA$\rightarrow$PEMS-BAY}} & \multicolumn{6}{c}{\textbf{PEMS-BAY$\rightarrow$METR-LA}}\\
% \cmidrule{2-7}
% \cmidrule{8-13}
\cline{2-7}
\cline{8-13}
& \multicolumn{2}{c}{5 min} & \multicolumn{2}{c}{15 min} & \multicolumn{2}{c||}{30 min}& \multicolumn{2}{c}{5 min} & \multicolumn{2}{c}{15 min} & \multicolumn{2}{c}{30 min}\\
\cline{2-7}
\cline{8-13}
 &MAPE(\%) & MAE & MAPE(\%) & MAE & MAPE(\%)  & MAE & MAPE(\%) & MAE & MAPE(\%) & MAE & MAPE(\%)  & MAE\\ 

\midrule
\midrule
STEP&  2.386$\pm$0.176 & 1.174$\pm$0.004 & 3.699$\pm$0.194 & 1.751$\pm$0.024 & 5.291$\pm$0.162  &2.363$\pm$0.038 & 7.230$\pm$1.180 & 2.737$\pm$0.127 &9.317$\pm$0.340 &3.317$\pm$0.008  &11.885$\pm$0.542 &4.147$\pm$0.260\\ 
  
3STEP+M+E & 2.560$\pm$0.158 & 1.314$\pm$0.094 & 3.937$\pm$0.097 & 1.952$\pm$0.050 & 5.787$\pm$0.171 & 2.800$\pm$0.19 & 6.348$\pm$0.181 & 2.746$\pm$0.090 & 8.908$\pm$0.203 & 3.473$\pm$0.073 & 11.784$\pm$0.238 & 4.428$\pm$0.12
\\

CROSS+M+E & 2.769$\pm$0.145 & 1.374$\pm$0.061 & 4.074$\pm$0.141 & 1.989$\pm$0.054 & 5.810$\pm$0.285 & 2.776$\pm$0.20 & 6.248$\pm$0.072 & 2.642$\pm$0.057 & 8.733$\pm$0.111 & 3.382$\pm$0.078 & 11.356$\pm$0.157 & 4.274$\pm$0.06
\\ 

CROSS+S+M+E & 2.614$\pm$0.179 & 1.288$\pm$0.068 & 3.969$\pm$0.158 & 1.877$\pm$0.055 & 5.585$\pm$0.160 & 2.512$\pm$0.06 & 6.087$\pm$0.192 & 2.567$\pm$0.048 & 8.537$\pm$0.375 & 3.312$\pm$0.059 & 11.305$\pm$0.461 & 4.250$\pm$0.03
\\

STEP+M &2.792$\pm$0.612 & 1.296$\pm$0.142 & 3.947$\pm$0.504 & 1.816$\pm$0.092 & 5.307$\pm$0.429 & 2.375$\pm$0.055 &6.440$\pm$0.378 & 2.708$\pm$0.090 & 8.491$\pm$0.420 & 3.364$\pm$0.074 & 10.885$\pm$0.342 & 4.150$\pm$0.117  \\ 

STEP+M+E & 2.407$\pm$0.114 & 1.198$\pm$0.010 & 3.628$\pm$0.110 & 1.761$\pm$0.017 & 5.084$\pm$0.072 & 2.341$\pm$0.037 &6.377$\pm$0.154 & 2.661$\pm$0.029 & 8.732$\pm$0.239 & 3.385$\pm$0.024 & 11.282$\pm$0.363 & 4.161$\pm$0.069
 
 \\ 
CROSS+S+C & 2.148$\pm$0.093 & 1.111$\pm$0.040 & 3.802$\pm$0.123 & 1.842$\pm$0.025 & 5.422$\pm$0.050 & 2.510$\pm$0.055 &6.132$\pm$0.147 & 2.581$\pm$0.028 & 8.799$\pm$0.378 & 3.337$\pm$0.057 & 11.487$\pm$0.481 & 4.242$\pm$0.125

  \\ 
CROSS+S+C+M & 2.168$\pm$0.066 & 1.130$\pm$0.037 & 3.664$\pm$0.106 & 1.817$\pm$0.043 & 5.282$\pm$0.248 & 2.453$\pm$0.087& 5.968$\pm$0.163 & 2.518$\pm$0.049 & 8.394$\pm$0.234 & 3.257$\pm$0.120 & 11.160$\pm$0.265 & 4.165$\pm$0.174
 
  \\ 



\midrule
FEPCross&  1.984$\pm$0.018 & 1.044$\pm$0.010 & 3.483$\pm$0.037 & 1.706$\pm$0.014 & 5.038$\pm$0.067 & 2.313$\pm$0.023 & 6.039$\pm$0.140 & 2.494$\pm$0.021 & 8.800$\pm$0.181 & 3.228$\pm$0.007 & 11.409$\pm$0.195 & 4.010$\pm$0.052 \\ 

\midrule
\midrule
& \multicolumn{6}{c||}{\textbf{Shenzhen$\rightarrow$Chengdu}} & \multicolumn{6}{c}{\textbf{Chengdu$\rightarrow$Shenzhen}}\\
\cline{2-7}
\cline{8-13}
& \multicolumn{2}{c}{10 min} & \multicolumn{2}{c}{30 min} & \multicolumn{2}{c||}{60 min}& \multicolumn{2}{c}{10 min} & \multicolumn{2}{c}{30 min} & \multicolumn{2}{c}{60 min}\\
\cline{2-7}
\cline{8-13}
 &MAPE(\%) & MAE & MAPE(\%) & MAE & MAPE(\%)  & MAE & MAPE(\%) & MAE & MAPE(\%) & MAE & MAPE(\%)  & MAE\\ 
\midrule
\midrule
STEP&  9.211$\pm$0.124 & 2.314$\pm$0.032 & 12.057$\pm$0.013 &2.883$\pm$0.044 &13.300$\pm$0.106  &3.167$\pm$0.043 & 7.616$\pm$0.085 & 1.954$\pm$0.001 &9.917$\pm$0.182 & 2.435$\pm$0.023 &10.883$\pm$0.137 &2.721$\pm$0.068\\ 

3STEP+M+E & 9.314$\pm$0.129 & 2.244$\pm$0.017 & 11.873$\pm$0.102 & 2.754$\pm$0.017 & 12.854$\pm$0.132 & 2.957$\pm$0.03 & 7.933$\pm$0.073 & 2.071$\pm$0.028 & 10.137$\pm$0.125 & 2.591$\pm$0.052 & 10.986$\pm$0.013 & 2.824$\pm$0.01
  \\ 
  
CROSS+M+E & 9.189$\pm$0.047 & 2.221$\pm$0.023 & 11.636$\pm$0.100 & 2.690$\pm$0.018 & 12.391$\pm$0.092 & 2.857$\pm$0.02 & 7.639$\pm$0.086 & 1.982$\pm$0.028 & 9.670$\pm$0.092 & 2.478$\pm$0.045 & 10.228$\pm$0.133 & 2.613$\pm$0.05
  \\ 

CROSS+S+M+E & 9.083$\pm$0.055 & 2.193$\pm$0.014 & 11.651$\pm$0.116 & 2.669$\pm$0.020 & 12.490$\pm$0.107 & 2.857$\pm$0.03 & 7.743$\pm$0.063 & 1.998$\pm$0.026 & 9.787$\pm$0.091 & 2.471$\pm$0.030 & 10.440$\pm$0.108 & 2.614$\pm$0.04
\\
  
STEP+M &9.928$\pm$0.341 & 2.337$\pm$0.054 & 12.541$\pm$0.176 & 2.812$\pm$0.005 & 14.056$\pm$0.395 & 3.122$\pm$0.073&8.100$\pm$0.090 & 2.098$\pm$0.025 & 9.990$\pm$0.110 & 2.523$\pm$0.056 & 10.400$\pm$0.084 & 2.624$\pm$0.042  \\ 

STEP+M+E & 9.578$\pm$0.134 & 2.308$\pm$0.041 & 12.491$\pm$0.114 & 2.848$\pm$0.024 & 13.880$\pm$0.283 & 3.136$\pm$0.052 &8.119$\pm$0.258 & 2.042$\pm$0.045 & 10.249$\pm$0.134 & 2.519$\pm$0.045 & 11.212$\pm$0.288 & 2.747$\pm$0.061
 
 \\ 
CROSS+S+C& 9.444$\pm$0.043 & 2.328$\pm$0.025 & 12.223$\pm$0.135 & 2.920$\pm$0.09 & 12.669$\pm$0.136 & 3.006$\pm$0.089 &7.613$\pm$0.036 & 1.958$\pm$0.017 & 9.665$\pm$0.073 & 2.456$\pm$0.037 & 10.098$\pm$0.125 & 2.572$\pm$0.053

  \\ 
CROSS+S+C+M & 8.886$\pm$0.065 & 2.161$\pm$0.008 & 11.552$\pm$0.132 & 2.664$\pm$0.006 & 12.152$\pm$0.043 & 2.783$\pm$0.015 & 7.392$\pm$0.044 & 1.874$\pm$0.014 & 9.337$\pm$0.040 & 2.324$\pm$0.040 & 9.893$\pm$0.079 & 2.461$\pm$0.027
 
  \\ 




\midrule
FEPCross&  8.941$\pm$0.087 & 2.160$\pm$0.013 & 11.419$\pm$0.123 & 2.631$\pm$0.024 & 12.042$\pm$0.053 & 2.779$\pm$0.010 & 7.345$\pm$0.048 & 1.892$\pm$0.031 & 9.261$\pm$0.082 & 2.317$\pm$0.042 & 9.811$\pm$0.070 & 2.455$\pm$0.027\\ 
\bottomrule
\bottomrule

\end{tabular}
}
% }
% \vspace{-.18cm}
\end{table*}

==> table/ablation_raw_table.tex <==
\begin{table*}[htb]
% \caption{Performance comparison between FDTI and baselines on four datasets. All attention based methods can not run on these large scale datasets and AGCRN, as can not run on the first three datasets due to the unrealistically huge memory consumption. Horizon means the number of forecasting steps.}
% \vspace{-.1cm}
\caption{Overall performance of few-shot traffic forecasting on \textit{PEMS-BAY}, \textit{METR-LA}, \textit{Chengdu}, and \textit{Shenzhen}. Metr-LA$\rightarrow$PEMS-BAY means the source data is METR-LA and the target data is PEMS-BAY. The mean and standard deviation of the results in 5 runs is shown. In each column, the best result is highlighted in bold and grey, and the second-best result is underlined. Marker * and ** indicates the mean of the results is statistically significant  (* means t-test with p-value $<$ 0.05 and ** means t-test with p-value $<$ 0.01). M means using momentum method to update adjacency matrix for STmodel. S means using spatial layer in transformer encoder. E means using augmented data during finetuning. C means using contrastive loss in pretrain.}
\label{tab:ablation_bkp}
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{c|c c|c c|c c||c c|c c|c c}
\resizebox{0.99\linewidth}{!}{

\begin{tabular}{c|c c c c c c||c c c c c c}
\toprule
& \multicolumn{6}{c||}{\textbf{METR-LA$\rightarrow$PEMS-BAY}} & \multicolumn{6}{c}{\textbf{PEMS-BAY$\rightarrow$METR-LA}}\\
% \cmidrule{2-7}
% \cmidrule{8-13}
\cline{2-7}
\cline{8-13}
& \multicolumn{2}{c}{5 min} & \multicolumn{2}{c}{15 min} & \multicolumn{2}{c||}{30 min}& \multicolumn{2}{c}{5 min} & \multicolumn{2}{c}{15 min} & \multicolumn{2}{c}{30 min}\\
\cline{2-7}
\cline{8-13}
 &MAPE(\%) & MAE & MAPE(\%) & MAE & MAPE(\%)  & MAE & MAPE(\%) & MAE & MAPE(\%) & MAE & MAPE(\%)  & MAE\\ 

\midrule
\midrule
STEP&  2.386$\pm$0.176 & 1.174$\pm$0.004 & 3.699$\pm$0.194 & 1.751$\pm$0.024 & 5.291$\pm$0.162  &2.363$\pm$0.038 & 7.230$\pm$1.180 & 2.737$\pm$0.127 &9.317$\pm$0.340 &3.317$\pm$0.008  &11.885$\pm$0.542 &4.147$\pm$0.260\\ 

STEP+M &2.792$\pm$0.612 & 1.296$\pm$0.142 & 3.947$\pm$0.504 & 1.816$\pm$0.092 & 5.307$\pm$0.429 & 2.375$\pm$0.055 &6.440$\pm$0.378 & 2.708$\pm$0.090 & 8.491$\pm$0.420 & 3.364$\pm$0.074 & 10.885$\pm$0.342 & 4.150$\pm$0.117  \\ 

STEP+M+E & 2.407$\pm$0.114 & 1.198$\pm$0.010 & 3.628$\pm$0.110 & 1.761$\pm$0.017 & 5.084$\pm$0.072 & 2.341$\pm$0.037 &6.377$\pm$0.154 & 2.661$\pm$0.029 & 8.732$\pm$0.239 & 3.385$\pm$0.024 & 11.282$\pm$0.363 & 4.161$\pm$0.069
 
 \\ 
CROSS+S+C & 2.148$\pm$0.093 & 1.111$\pm$0.040 & 3.802$\pm$0.123 & 1.842$\pm$0.025 & 5.422$\pm$0.050 & 2.510$\pm$0.055 &6.132$\pm$0.147 & 2.581$\pm$0.028 & 8.799$\pm$0.378 & 3.337$\pm$0.057 & 11.487$\pm$0.481 & 4.242$\pm$0.125

  \\ 
CROSS+S+C+M & 2.168$\pm$0.066 & 1.130$\pm$0.037 & 3.664$\pm$0.106 & 1.817$\pm$0.043 & 5.282$\pm$0.248 & 2.453$\pm$0.087& 5.968$\pm$0.163 & 2.518$\pm$0.049 & 8.394$\pm$0.234 & 3.257$\pm$0.120 & 11.160$\pm$0.265 & 4.165$\pm$0.174
 
  \\ 
3STEP+M+E & 2.560$\pm$0.158 & 1.314$\pm$0.094 & 3.937$\pm$0.097 & 1.952$\pm$0.050 & 5.787$\pm$0.171 & 2.800$\pm$0.19 & 6.348$\pm$0.181 & 2.746$\pm$0.090 & 8.908$\pm$0.203 & 3.473$\pm$0.073 & 11.784$\pm$0.238 & 4.428$\pm$0.12
  \\ 
CROSS+M+E & 2.769$\pm$0.145 & 1.374$\pm$0.061 & 4.074$\pm$0.141 & 1.989$\pm$0.054 & 5.810$\pm$0.285 & 2.776$\pm$0.20 & 6.248$\pm$0.072 & 2.642$\pm$0.057 & 8.733$\pm$0.111 & 3.382$\pm$0.078 & 11.356$\pm$0.157 & 4.274$\pm$0.06
  \\ 
CROSS+S+M+E & 2.614$\pm$0.179 & 1.288$\pm$0.068 & 3.969$\pm$0.158 & 1.877$\pm$0.055 & 5.585$\pm$0.160 & 2.512$\pm$0.06 & 6.087$\pm$0.192 & 2.567$\pm$0.048 & 8.537$\pm$0.375 & 3.312$\pm$0.059 & 11.305$\pm$0.461 & 4.250$\pm$0.03
\\

\midrule
FEPCross&  1.984$\pm$0.018 & 1.044$\pm$0.010 & 3.483$\pm$0.037 & 1.706$\pm$0.014 & 5.038$\pm$0.067 & 2.313$\pm$0.023 & 6.039$\pm$0.140 & 2.494$\pm$0.021 & 8.800$\pm$0.181 & 3.228$\pm$0.007 & 11.409$\pm$0.195 & 4.010$\pm$0.052 \\ 

\midrule
\midrule
& \multicolumn{6}{c||}{\textbf{Shenzhen$\rightarrow$Chengdu}} & \multicolumn{6}{c}{\textbf{Chengdu$\rightarrow$Shenzhen}}\\
\cline{2-7}
\cline{8-13}
& \multicolumn{2}{c}{10 min} & \multicolumn{2}{c}{30 min} & \multicolumn{2}{c||}{60 min}& \multicolumn{2}{c}{10 min} & \multicolumn{2}{c}{30 min} & \multicolumn{2}{c}{60 min}\\
\cline{2-7}
\cline{8-13}
 &MAPE(\%) & MAE & MAPE(\%) & MAE & MAPE(\%)  & MAE & MAPE(\%) & MAE & MAPE(\%) & MAE & MAPE(\%)  & MAE\\ 
\midrule
\midrule
STEP&  9.211$\pm$0.124 & 2.314$\pm$0.032 & 12.057$\pm$0.013 &2.883$\pm$0.044 &13.300$\pm$0.106  &3.167$\pm$0.043 & 7.616$\pm$0.085 & 1.954$\pm$0.001 &9.917$\pm$0.182 & 2.435$\pm$0.023 &10.883$\pm$0.137 &2.721$\pm$0.068\\ 

STEP+M &9.928$\pm$0.341 & 2.337$\pm$0.054 & 12.541$\pm$0.176 & 2.812$\pm$0.005 & 14.056$\pm$0.395 & 3.122$\pm$0.073&8.100$\pm$0.090 & 2.098$\pm$0.025 & 9.990$\pm$0.110 & 2.523$\pm$0.056 & 10.400$\pm$0.084 & 2.624$\pm$0.042  \\ 

STEP+M+E & 9.578$\pm$0.134 & 2.308$\pm$0.041 & 12.491$\pm$0.114 & 2.848$\pm$0.024 & 13.880$\pm$0.283 & 3.136$\pm$0.052 &8.119$\pm$0.258 & 2.042$\pm$0.045 & 10.249$\pm$0.134 & 2.519$\pm$0.045 & 11.212$\pm$0.288 & 2.747$\pm$0.061
 
 \\ 
CROSS+S+C& 9.444$\pm$0.043 & 2.328$\pm$0.025 & 12.223$\pm$0.135 & 2.920$\pm$0.09 & 12.669$\pm$0.136 & 3.006$\pm$0.089 &7.613$\pm$0.036 & 1.958$\pm$0.017 & 9.665$\pm$0.073 & 2.456$\pm$0.037 & 10.098$\pm$0.125 & 2.572$\pm$0.053

  \\ 
CROSS+S+C+M & 8.886$\pm$0.065 & 2.161$\pm$0.008 & 11.552$\pm$0.132 & 2.664$\pm$0.006 & 12.152$\pm$0.043 & 2.783$\pm$0.015 & 7.392$\pm$0.044 & 1.874$\pm$0.014 & 9.337$\pm$0.040 & 2.324$\pm$0.040 & 9.893$\pm$0.079 & 2.461$\pm$0.027
 
  \\ 
3STEP+M+E & 9.314$\pm$0.129 & 2.244$\pm$0.017 & 11.873$\pm$0.102 & 2.754$\pm$0.017 & 12.854$\pm$0.132 & 2.957$\pm$0.03 & 7.933$\pm$0.073 & 2.071$\pm$0.028 & 10.137$\pm$0.125 & 2.591$\pm$0.052 & 10.986$\pm$0.013 & 2.824$\pm$0.01
  \\ 
CROSS+M+E & 9.189$\pm$0.047 & 2.221$\pm$0.023 & 11.636$\pm$0.100 & 2.690$\pm$0.018 & 12.391$\pm$0.092 & 2.857$\pm$0.02 & 7.639$\pm$0.086 & 1.982$\pm$0.028 & 9.670$\pm$0.092 & 2.478$\pm$0.045 & 10.228$\pm$0.133 & 2.613$\pm$0.05
  \\ 
CROSS+S+M+E & 9.083$\pm$0.055 & 2.193$\pm$0.014 & 11.651$\pm$0.116 & 2.669$\pm$0.020 & 12.490$\pm$0.107 & 2.857$\pm$0.03 & 7.743$\pm$0.063 & 1.998$\pm$0.026 & 9.787$\pm$0.091 & 2.471$\pm$0.030 & 10.440$\pm$0.108 & 2.614$\pm$0.04
\\


\midrule
FEPCross&  8.941$\pm$0.087 & 2.160$\pm$0.013 & 11.419$\pm$0.123 & 2.631$\pm$0.024 & 12.042$\pm$0.053 & 2.779$\pm$0.010 & 7.345$\pm$0.048 & 1.892$\pm$0.031 & 9.261$\pm$0.082 & 2.317$\pm$0.042 & 9.811$\pm$0.070 & 2.455$\pm$0.027\\ 
\bottomrule
\bottomrule

\end{tabular}
}
% }
% \vspace{-.18cm}
\end{table*}

==> table/crosscity_bkp.tex <==
\begin{table*}[!th]
% \caption{Performance comparison between FDTI and baselines on four datasets. All attention based methods can not run on these large scale datasets and AGCRN, as can not run on the first three datasets due to the unrealistically huge memory consumption. Horizon means the number of forecasting steps.}
% \vspace{-.1cm}
\caption{Overall performance of few-shot traffic forecasting on \textit{PEMS-BAY}, \textit{METR-LA}, \textit{Chengdu}, and \textit{Shenzhen}. Metr-LA$\rightarrow$PEMS-BAY means the source data is METR-LA and the target data is PEMS-BAY. The mean and standard deviation of the results in 5 runs is shown. In each column, the best result is highlighted in bold and grey, and the second-best result is underlined. Marker * and ** indicates the mean of the results is statistically significant  (* means t-test with p-value $<$ 0.05 and ** means t-test with p-value $<$ 0.01).}
\label{tab:performance}
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{c|c c|c c|c c||c c|c c|c c}
\resizebox{0.99\linewidth}{!}{

\begin{tabular}{c|c c c c c c||c c c c c c}
\toprule
& \multicolumn{6}{c||}{\textbf{METR-LA$\rightarrow$PEMS-BAY}} & \multicolumn{6}{c}{\textbf{PEMS-BAY$\rightarrow$METR-LA}}\\
% \cmidrule{2-7}
% \cmidrule{8-13}
\cline{2-7}
\cline{8-13}
& \multicolumn{2}{c}{5 min} & \multicolumn{2}{c}{15 min} & \multicolumn{2}{c||}{30 min}& \multicolumn{2}{c}{5 min} & \multicolumn{2}{c}{15 min} & \multicolumn{2}{c}{30 min}\\
\cline{2-7}
\cline{8-13}
 &MAPE(\%) & MAE & MAPE(\%) & MAE & MAPE(\%)  & MAE & MAPE(\%) & MAE & MAPE(\%) & MAE & MAPE(\%)  & MAE\\ 

\midrule
\midrule
HA & 9.333 & 3.993 & 9.333 & 3.993  & 9.333 & 3.993 & 14.152 & 5.206 &  14.152 & 5.206 & 14.152 & 5.206 \\ 
SVR&  8.074 & 3.789 & 7.958 & 3.695 & 7.952 & 3.705 & 14.024 & 4.967  &14.587 & 5.108 & 14.024& 5.037 \\ 
\midrule
DCRNN & 3.661$\pm$0.212 & 1.642$\pm$0.041 & 4.450$\pm$0.212 & 2.038$\pm$0.057 & 5.795$\pm$0.151 & 2.658$\pm$0.055 & 7.879$\pm$0.214 & 3.129$\pm$0.142 & 9.427$\pm$0.250 & 3.555$\pm$0.106 & 11.907$\pm$0.416 & 4.306$\pm$0.175 

 \\ 
GWN & 3.672$\pm$0.702 & 1.485$\pm$0.179 & 5.142$\pm$0.761 & 2.065$\pm$0.161 & 7.042$\pm$1.038 & 2.718$\pm$0.226 & 6.666$\pm$0.476 & 2.775$\pm$0.080 & 9.825$\pm$0.801 & 3.492$\pm$0.154 & 12.774$\pm$1.073 & 4.355$\pm$0.206 

 \\ 
STFGNN & 3.214$\pm$0.504 & 1.485$\pm$0.112 & 4.051$\pm$0.166 & 1.925$\pm$0.061 & 5.683$\pm$0.177 & 2.656$\pm$0.128 & 7.570$\pm$0.463 & 3.398$\pm$0.320 & 9.784$\pm$0.422 & 3.925$\pm$0.201 & 12.496$\pm$0.648 & 4.517$\pm$0.249 

  \\ 
DSTAGNN & 3.360$\pm$0.488 & 1.670$\pm$0.319 & 4.797$\pm$0.803 & 2.338$\pm$0.540 & 6.285$\pm$0.664 & 2.852$\pm$0.374 & 7.113$\pm$0.571 & 2.824$\pm$0.141 & 10.184$\pm$1.227 & 3.589$\pm$0.468 & 12.558$\pm$1.110 & 4.418$\pm$0.372 

  \\ 
FOGS & 2.872$\pm$0.283 & 1.382$\pm$0.077 & 3.938$\pm$0.236 & 1.866$\pm$0.054 & 5.635$\pm$0.303 & 2.618$\pm$0.059  & 7.203$\pm$0.434 & 3.229$\pm$0.294 & 9.557$\pm$0.553 & 3.837$\pm$0.253 & 12.411$\pm$0.626 & 4.480$\pm$0.248 


  \\ 
DLinear&2.640$\pm$0.214 & 1.441$\pm$0.136 & 4.042$\pm$0.143 & 2.086$\pm$0.065 & 5.637$\pm$0.463 & 2.801$\pm$0.238 & 6.628$\pm$0.307 & 2.844$\pm$0.058 & 9.335$\pm$0.687 & 3.664$\pm$0.224 & 11.869$\pm$0.421 & 4.465$\pm$0.102 
\\
FEDFormer & 6.012$\pm$0.548 & 3.078$\pm$0.365 & 5.874$\pm$0.512 & 2.894$\pm$0.238 & 5.648$\pm$0.457 & 2.691$\pm$0.238 &  14.349$\pm$0.915 & 5.019$\pm$0.402& 13.124$\pm$0.997 & 4.978$\pm$0.352& 12.236$\pm$0.343 & 4.789$\pm$0.402
\\

ST-GFSL& 2.878$\pm$0.135 & 1.384$\pm$0.037  & 4.124$\pm$0.078 & 1.987$\pm$0.046 & 5.458$\pm$0.153  &2.475$\pm$0.089 &7.014$\pm$0.045 &2.798$\pm$0.034 &9.174$\pm$0.106 &3.432$\pm$0.078  &13.474$\pm$0.677 &4.445$\pm$0.157  \\ 
STEP&  2.386$\pm$0.176 & 1.174$\pm$0.004 & 3.699$\pm$0.194 & 1.751$\pm$0.024 & 5.291$\pm$0.162  &2.363$\pm$0.038 & 7.230$\pm$1.180 & 2.737$\pm$0.127 &9.317$\pm$0.340 &3.317$\pm$0.008  &11.885$\pm$0.542 &4.147$\pm$0.260\\ 

TransGTR & 3.615$\pm$0.135 & 1.470$\pm$0.033 & 4.510$\pm$0.168 &  1.891$\pm$0.024 & 5.572$\pm$0.201  &2.353$\pm$0.036 & 7.726$\pm$0.075 & 2.860$\pm$0.077 &8.993$\pm$0.116 &3.314$\pm$0.032  &11.510$\pm$0.607 &4.074$\pm$0.040\\ 

TPB & 2.547$\pm$0.293 & 1.186$\pm$0.077 & 3.864$\pm$0.287 & 1.700$\pm$0.065 & 5.434$\pm$0.313 & 2.359$\pm$0.061 & 6.611$\pm$0.110 &  2.781$\pm$0.159 & 8.971$\pm$0.643 & 3.294$\pm$0.102 & 11.970$\pm$1.108 & 3.975$\pm$0.089  \\ 

\midrule
FEPCross&  1.984$\pm$0.018 & 1.044$\pm$0.010 & 3.483$\pm$0.037 & 1.706$\pm$0.014 & 5.038$\pm$0.067 & 2.313$\pm$0.023 & 6.039$\pm$0.140 & 2.494$\pm$0.021 & 8.800$\pm$0.181 & 3.228$\pm$0.007 & 11.409$\pm$0.195 & 4.010$\pm$0.052 \\ 

\midrule
\midrule
& \multicolumn{6}{c||}{\textbf{Shenzhen$\rightarrow$Chengdu}} & \multicolumn{6}{c}{\textbf{Chengdu$\rightarrow$Shenzhen}}\\
\cline{2-7}
\cline{8-13}
& \multicolumn{2}{c}{10 min} & \multicolumn{2}{c}{30 min} & \multicolumn{2}{c||}{60 min}& \multicolumn{2}{c}{10 min} & \multicolumn{2}{c}{30 min} & \multicolumn{2}{c}{60 min}\\
\cline{2-7}
\cline{8-13}
 &MAPE(\%) & MAE & MAPE(\%) & MAE & MAPE(\%)  & MAE & MAPE(\%) & MAE & MAPE(\%) & MAE & MAPE(\%)  & MAE\\ 
\midrule
\midrule
HA & 16.273 & 3.770 & 16.273 & 3.770  & 16.273 & 3.770 & 17.325 & 4.431 & 17.325 & 4.431 & 17.325 & 4.431 \\ 
SVR & 15.387 & 3.578  & 15.566 & 3.620  & 15.789 & 3.709 & 15.014 & 4.019 & 15.678  & 4.168 & 16.115 & 4.348 \\ 
\midrule
DCRNN & 10.383$\pm$0.244 & 2.554$\pm$0.021 & 14.069$\pm$0.311 & 3.233$\pm$0.030 & 15.259$\pm$0.226 & 3.551$\pm$0.037 & 8.258$\pm$0.148 & 2.187$\pm$0.046 & 10.664$\pm$0.089 & 2.695$\pm$0.035 & 11.388$\pm$0.212 & 2.952$\pm$0.058 

 \\ 
GWN & 10.487$\pm$0.629 & 2.571$\pm$0.070 & 14.739$\pm$0.985 & 3.359$\pm$0.110 & 15.815$\pm$0.825 & 3.699$\pm$0.062 & 8.622$\pm$0.293 & 2.250$\pm$0.041 & 11.464$\pm$0.443 & 2.875$\pm$0.080 & 12.212$\pm$0.547 & 3.151$\pm$0.111 

  \\ 
STFGNN & 11.790$\pm$0.855 & 2.904$\pm$0.112 & 15.775$\pm$0.977 & 3.594$\pm$0.093 & 16.950$\pm$0.851 & 3.951$\pm$0.070 & 9.960$\pm$0.540 & 2.554$\pm$0.077 & 12.600$\pm$0.808 & 3.091$\pm$0.098 & 13.208$\pm$0.742 & 3.352$\pm$0.086 

  \\ 
DSTAGNN & 10.373$\pm$0.391 & 2.550$\pm$0.041 & 15.313$\pm$1.146 & 3.458$\pm$0.308 & 15.469$\pm$0.884 & 3.616$\pm$0.100 & 9.273$\pm$0.998 & 2.478$\pm$0.322 & 11.939$\pm$0.797 & 2.938$\pm$0.145 & 13.174$\pm$1.179 & 3.408$\pm$0.428 

  \\ 
FOGS & 11.626$\pm$0.822 & 2.834$\pm$0.101 & 15.787$\pm$0.993 & 3.561$\pm$0.107 & 16.894$\pm$0.988 & 3.905$\pm$0.103 & 9.322$\pm$0.128 & 2.439$\pm$0.021 & 12.001$\pm$0.198 & 3.013$\pm$0.028 & 12.640$\pm$0.179 & 3.278$\pm$0.051 
  \\ 
DLinear & 10.756$\pm$0.082 & 2.719$\pm$0.022 & 14.150$\pm$0.268 & 3.397$\pm$0.072 & 13.981$\pm$0.317 & 3.451$\pm$0.090 & 8.791$\pm$0.063 & 2.349$\pm$0.012 & 11.074$\pm$0.078 & 2.851$\pm$0.035 & 11.199$\pm$0.115 & 3.001$\pm$0.053 
\\
FEDFormer & 13.987$\pm$0.756 & 3.255$\pm$0.173 & 13.527$\pm$0.856 & 3.063$\pm$0.165 & 13.487$\pm$0.621 & 3.166$\pm$0.190 & 11.879$\pm$0.874 & 2.868$\pm$0.289 & 11.548$\pm$0.697 & 2.756$\pm$0.306 & 11.648$\pm$0.354 & 2.778$\pm$0.225 \\
ST-GFSL& 9.729$\pm$0.478 & 2.397$\pm$0.061 & 12.914$\pm$0.884 &2.942$\pm$0.107 &14.259$\pm$1.025  &3.349$\pm$0.109 & 8.240$\pm$0.554 &2.035$\pm$0.034 &10.672$\pm$0.889 & 2.459$\pm$0.067 &11.910$\pm$1.003 &2.781$\pm$0.097  \\ 

STEP&  9.211$\pm$0.124 & 2.314$\pm$0.032 & 12.057$\pm$0.013 &2.883$\pm$0.044 &13.300$\pm$0.106  &3.167$\pm$0.043 & 7.616$\pm$0.085 & 1.954$\pm$0.001 &9.917$\pm$0.182 & 2.435$\pm$0.023 &10.883$\pm$0.137 &2.721$\pm$0.068\\ 

TransGTR& 9.510$\pm$0.129 & 2.277$\pm$0.036 & 12.235$\pm$0.181 &2.791$\pm$0.019 &13.376$\pm$0.171  &3.024$\pm$0.032 & 7.942$\pm$0.087 & 2.038$\pm$0.035 &9.834$\pm$0.080 & 2.456$\pm$0.038 &10.601$\pm$0.044 &2.636$\pm$0.030\\ 

TPB & 9.180$\pm$0.130 & 2.192$\pm$0.020 &  12.096$\pm$0.187 & 2.752$\pm$0.035 & 13.207$\pm$0.266 & 3.020$\pm$0.037 & 7.613$\pm$0.130 & 1.944$\pm$0.065 & 9.965$\pm$0.162 & 2.384$\pm$0.084 & 10.570$\pm$0.197 & 2.684$\pm$0.078 \\ 

\midrule
FEPCross& 8.941$\pm$0.087 & 2.160$\pm$0.013 & 11.419$\pm$0.123 & 2.631$\pm$0.024 & 12.042$\pm$0.053 & 2.779$\pm$0.010 & 7.345$\pm$0.048 & 1.892$\pm$0.031 & 9.261$\pm$0.082 & 2.317$\pm$0.042 & 9.811$\pm$0.070 & 2.455$\pm$0.027 \\ 
\bottomrule
\bottomrule

\end{tabular}
}
% }
% \vspace{-.18cm}
\end{table*}
